Accelerating Neural Network Training: An Analysis of the AlgoPerf Competition

The goal of the AlgoPerf: Training Algorithms competition is to evaluate practical speed-ups in neural network training achieved solely by improving the underlying training algorithms. In the external tuning ruleset, submissions must provide workload-agnostic hyperparameter search spaces, while in the self-tuning ruleset they must be completely hyperparameter-free. In both rulesets, submissions are compared on time-to-result across multiple deep learning workloads, training on fixed hardware. This paper presents the inaugural AlgoPerf competition's results, which drew 18 diverse submissions from 10 teams. Our investigation reveals several key findings: (1) The winning submission in the external tuning ruleset, using Distributed Shampoo, demonstrates the effectiveness of non-diagonal preconditioning over popular methods like Adam, even when compared on wall-clock runtime. (2) The winning submission in the self-tuning ruleset, based on the Schedule Free AdamW algorithm, demonstrates a new level of effectiveness for completely hyperparameter-free training algorithms. (3) The top-scoring submissions were surprisingly robust to workload changes. We also discuss the engineering challenges encountered in ensuring a fair comparison between different training algorithms. These results highlight both the significant progress so far, and the considerable room for further improvements.

==> figs/held_out_workloads.tex <==

\begin{tabularx}{0.98\textwidth}{@{}XllS[table-format=2.6]S[table-format=6.0]@{}}
	\toprule
                              &                  &                             & {Validation}      & {Runtime}         \\ 
\textbf{Task}                 & \textbf{Dataset} & \textbf{Variant}            & \textbf{Target}   & \textbf{Budget} \\ \midrule
Clickthrough rate prediction  & \criteo          & \textsc{Embed Init Scale}     & 0.129657        & 7703              \\ \addlinespace
MRI reconstruction            & \fastmri         & \textsc{TanH}                 & 0.717840          & 8859              \\ \addlinespace
Image classification          & \imagenet        & \textsc{ResNet BN Init Scale} & 0.23474         & 63008             \\ \addlinespace
Speech recognition            & \librispeech     & \textsc{Conformer LayerNorm}  & 0.09731         & 61068             \\ \addlinespace
Molecular property prediction & \ogbg            & \textsc{Altered Layers}       & 0.269446         & 18477             \\ \addlinespace
Translation                   & \wmt             & \textsc{GLU \& TanH}          & 29.5779         & 48151             \\ \bottomrule
\end{tabularx}


==> figs/leaderboard_external_tuning.tex <==
{\renewcommand{\arraystretch}{1.1}
  \setlength{\tabcolsep}{4pt}
  \hyphenpenalty=10000\exhyphenpenalty=10000
  \begin{tabularx}{\textwidth}{>{\raggedright\arraybackslash}XcS[table-format=1.4]}
    \toprule
    \textbf{Submission} & \textbf{Line} & \textbf{Score} \\ \midrule
    \shampoosub & \shampoosubline & 0.7784 \\
    \sfadam & \sfadamline & 0.7077 \\
    \generalizedadam & \generalizedadamline & 0.6383 \\
    \cycliclr & \cycliclrline & 0.6301 \\
    \nadamp & \nadampline & 0.5909 \\
    \rowcolor{TUgray_light}\baseline & \baselineline & 0.5707 \\
    \amos & \amosline & 0.4918 \\
    \caspr & \casprline & 0.4722 \\
    \lawaq & \lawaqline & 0.3699 \\
    \lawaema & \lawaemaline & 0.3384 \\
    \sfprodigy & \sfprodigyline & 0 \\
    \bottomrule
  \end{tabularx}
\vspace{0pt}}


==> figs/leaderboard_ignoring_wls_external_tuning.tex <==
{\renewcommand{\arraystretch}{1.25}
\setlength{\tabcolsep}{4pt}
\begin{tabularx}{0.99\textwidth}{@{}p{1.9cm}S[table-format=1.2]gS[table-format=1.2]gS[table-format=1.2]gS[table-format=1.2]gS[table-format=1.2]gS[table-format=1.2]gS[table-format=1.2]gS[table-format=1.2]gS[table-format=1.2]g@{}}
\toprule
 & \multicolumn{2}{c}{Full} & \multicolumn{2}{c}{\makecell{\textsc{Criteo}\\ \textsc{1TB}}} & \multicolumn{2}{c}{\fastmri} & \multicolumn{2}{c}{\resnet} & \multicolumn{2}{c}{\vit} & \multicolumn{2}{c}{\makecell{\textsc{Con-}\\ \textsc{former}}} & \multicolumn{2}{c}{\makecell{\textsc{Deep}\\ \textsc{Speech}}} & \multicolumn{2}{c}{\ogbg} & \multicolumn{2}{c}{\wmt} \\
 \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13} \cmidrule(lr){14-15} \cmidrule(lr){16-17} \cmidrule(lr){18-19}
 & \text{Score} & \text{Rank} & \text{S.} & \text{R.} & \text{S.} & \text{R.} & \text{S.} & \text{R.} & \text{S.} & \text{R.} & \text{S.} & \text{R.} & \text{S.} & \text{R.} & \text{S.} & \text{R.} & \text{S.} & \text{R.} \\
\midrule
\pytorch \textsc{Distr.} \newline \textsc{Shampoo} & 0.78 & 1 & 0.75 & 1 & 0.75 & 1 & 0.89 & 1 & 0.75 & 1 & 0.75 & 1 & 0.75 & 1 & 0.77 & 2 & 0.81 & 1 \\
\sfadam & 0.71 & 2 & 0.67 & 2 & 0.67 & 2 & 0.81 & 2 & 0.68 & 2 & 0.68 & 3 & 0.68 & 2 & 0.81 & 1 & 0.67 & 2 \\
\generalizedadam & 0.64 & 3 & 0.60 & 3 & 0.61 & 4 & 0.59 & 6 & 0.63 & 3 & 0.73 & 2 & 0.59 & 3 & 0.73 & 3 & 0.63 & 3 \\
\cycliclr & 0.63 & 4 & 0.58 & 4 & 0.62 & 3 & 0.72 & 3 & 0.62 & 4 & 0.59 & 4 & 0.59 & 4 & 0.72 & 4 & 0.60 & 4 \\
\nadamp & 0.59 & 5 & 0.54 & 6 & 0.57 & 5 & 0.68 & 4 & 0.58 & 5 & 0.55 & 5 & 0.53 & 5 & 0.68 & 5 & 0.60 & 5 \\
\baseline & 0.57 & 6 & 0.53 & 8 & 0.55 & 6 & 0.65 & 5 & 0.56 & 6 & 0.52 & 7 & 0.52 & 6 & 0.65 & 6 & 0.58 & 6 \\
\amos & 0.49 & 7 & 0.56 & 5 & 0.50 & 7 & 0.56 & 7 & 0.44 & 7 & 0.42 & 9 & 0.42 & 8 & 0.56 & 7 & 0.47 & 8 \\
\textsc{CASPR} \newline \textsc{Adaptive} & 0.47 & 8 & 0.54 & 7 & 0.40 & 8 & 0.54 & 8 & 0.41 & 8 & 0.54 & 6 & 0.41 & 9 & 0.40 & 8 & 0.54 & 7 \\
\lawaq & 0.37 & 9 & 0.42 & 9 & 0.32 & 9 & 0.42 & 9 & 0.31 & 9 & 0.42 & 8 & 0.42 & 7 & 0.33 & 10 & 0.31 & 10 \\
\lawaema & 0.34 & 10 & 0.25 & 10 & 0.31 & 10 & 0.39 & 10 & 0.28 & 10 & 0.39 & 10 & 0.39 & 10 & 0.39 & 9 & 0.32 & 9 \\
\sfprodigy & 0.00 & 11 & 0.00 & 11 & 0.00 & 11 & 0.00 & 11 & 0.00 & 11 & 0.00 & 11 & 0.00 & 11 & 0.00 & 11 & 0.00 & 11 \\
\bottomrule
\end{tabularx}
}


==> figs/leaderboard_ignoring_wls_self_tuning.tex <==
{\renewcommand{\arraystretch}{1.25}
\setlength{\tabcolsep}{4pt}
\begin{tabularx}{0.99\textwidth}{@{}p{1.9cm}S[table-format=1.2]gS[table-format=1.2]gS[table-format=1.2]gS[table-format=1.2]gS[table-format=1.2]gS[table-format=1.2]gS[table-format=1.2]gS[table-format=1.2]gS[table-format=1.2]g@{}}
\toprule
 & \multicolumn{2}{c}{Full} & \multicolumn{2}{c}{\makecell{\textsc{Criteo}\\ \textsc{1TB}}} & \multicolumn{2}{c}{\fastmri} & \multicolumn{2}{c}{\resnet} & \multicolumn{2}{c}{\vit} & \multicolumn{2}{c}{\makecell{\textsc{Con-}\\ \textsc{former}}} & \multicolumn{2}{c}{\makecell{\textsc{Deep}\\ \textsc{Speech}}} & \multicolumn{2}{c}{\ogbg} & \multicolumn{2}{c}{\wmt} \\
 \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13} \cmidrule(lr){14-15} \cmidrule(lr){16-17} \cmidrule(lr){18-19}
& \text{Score} & \text{Rank} & \text{S.} & \text{R.} & \text{S.} & \text{R.} & \text{S.} & \text{R.} & \text{S.} & \text{R.} & \text{S.} & \text{R.} & \text{S.} & \text{R.} & \text{S.} & \text{R.} & \text{S.} & \text{R.} \\
\midrule
\sfadam & 0.85 & 1 & 0.83 & 1 & 0.83 & 1 & 0.98 & 1 & 0.83 & 1 & 0.83 & 1 & 0.85 & 1 & 0.83 & 1 & 0.84 & 1 \\
\baseline & 0.82 & 2 & 0.79 & 2 & 0.82 & 2 & 0.94 & 2 & 0.81 & 2 & 0.79 & 2 & 0.79 & 2 & 0.81 & 2 & 0.79 & 2 \\
\textsc{NadamW}\newline \textsc{Sequential} & 0.33 & 3 & 0.38 & 3 & 0.27 & 3 & 0.38 & 3 & 0.30 & 3 & 0.38 & 3 & 0.29 & 3 & 0.27 & 3 & 0.38 & 3 \\
\sinvnum & 0.14 & 4 & 0.16 & 4 & 0.12 & 4 & 0.16 & 4 & 0.16 & 4 & 0.16 & 4 & 0.13 & 4 & 0.16 & 4 & 0.08 & 4 \\
\sinv & 0.09 & 5 & 0.10 & 5 & 0.07 & 5 & 0.10 & 5 & 0.10 & 5 & 0.10 & 5 & 0.09 & 5 & 0.10 & 5 & 0.04 & 5 \\
\adamg & 0.00 & 6\phantom{1} & 0.00 & 6\phantom{1} & 0.00 & 6\phantom{1} & 0.00 & 6\phantom{1} & 0.00 & 6\phantom{1} & 0.00 & 6\phantom{1} & 0.00 & 6 \phantom{1}& 0.00 & 6\phantom{1} & 0.00 & 6\phantom{1} \\
\bottomrule
\end{tabularx}
}


==> figs/leaderboard_self_tuning.tex <==
{\renewcommand{\arraystretch}{1.25}
  \setlength{\tabcolsep}{4pt}
  \hyphenpenalty=10000\exhyphenpenalty=10000
  \begin{tabularx}{\textwidth}{>{\raggedright\arraybackslash}XcS[table-format=1.4]}
    \toprule
    \textbf{Submission} & \textbf{Line} & \textbf{Score} \\ \midrule
    \sfadam & \sfadamline & 0.8542 \\
    \rowcolor{TUgray_light}\baseline & \baselineline & 0.8194 \\
    \nadamwseq & \nadamwseqline & 0.3308 \\
    \sinvnum & \sinvnumline & 0.1420 \\
    \sinv & \sinvline & 0.0903 \\
    \adamg & \adamgline & 0 \\
    \bottomrule
  \end{tabularx}
\vspace{3.33\baselineskip}
}


==> figs/runtimes_external_tuning.tex <==
{\renewcommand{\arraystretch}{1.25}\setlength{\tabcolsep}{4pt}\begin{tabularx}{0.99\textwidth}{>{\raggedright\arraybackslash}Xlglglgllgllglg}
\toprule
 & \multicolumn{2}{c}{\criteo} & \multicolumn{2}{c}{\fastmri} & \multicolumn{2}{c}{\resnet} & \vit & \multicolumn{2}{c}{\conformer} & \makecell{\textsc{Deep}\\ \textsc{Speech}} & \multicolumn{2}{c}{\ogbg} & \multicolumn{2}{c}{\wmt} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-8} \cmidrule(lr){9-10} \cmidrule(lr){11-11} \cmidrule(lr){12-13} \cmidrule(lr){14-15} & Base & H.O. & Base & H.O. & Base & H.O. & Base & Base & H.O. & Base & Base & H.O. & Base & H.O. \\
\midrule
\amos & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & 0.33 & 0.49 & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\B 0.55\textsuperscript{\textdagger}} & 0.65 & \B 0.71 & 0.57 & \B 0.57 & \textcolor{TUdark_light}{0.60\textsuperscript{\textasteriskcentered}} & \textcolor{TUdark_light}{0.89\textsuperscript{\textasteriskcentered}} & 0.68 & 0.37 \\
\baseline & 0.94 & 0.08 & 0.23 & 0.51 & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{0.94\textsuperscript{\textdagger}} & 0.91 & 0.90 & 0.83 & 0.65 & \textcolor{TUdark_light}{0.42\textsuperscript{\textdaggerdbl}} & \textcolor{TUdark_light}{0.68\textsuperscript{\textasteriskcentered}} & 0.86 & 0.35 \\
\textsc{CASPR} \newline \textsc{Adaptive} & \textcolor{TUdark_light}{\texttt{NaN}} & \textcolor{TUdark_light}{\texttt{NaN}} & \B 0.13 & \B 0.15 & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & 0.58 & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{0.59\textsuperscript{\textdagger}} & 0.75 & \B 0.12 & \B 0.12 & \textcolor{TUdark_light}{0.67\textsuperscript{\textdaggerdbl}} & \textcolor{TUdark_light}{\texttt{NaN}} \\
\cycliclr & 0.67 & 0.08 & 0.25 & 0.44 & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & 0.81 & 0.94 & 0.92 & 0.70 & \textcolor{TUdark_light}{0.38\textsuperscript{\textdaggerdbl}} & \textcolor{TUdark_light}{0.51\textsuperscript{\textasteriskcentered}} & 0.49 & 0.35 \\
\generalizedadam & 0.83 & 0.05 & 0.18 & 0.39 & \B 0.97 & 0.88 & 0.84 & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{0.83\textsuperscript{\textdagger}} & 0.68 & \textcolor{TUdark_light}{0.31\textsuperscript{\textdaggerdbl}} & \textcolor{TUdark_light}{0.64\textsuperscript{\textasteriskcentered}} & 0.63 & 0.33 \\
\lawaema & 0.69 & 0.09 & 0.29 & 0.57 & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & 0.80 & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{0.57\textsuperscript{\textasteriskcentered}} & \textcolor{TUdark_light}{0.73\textsuperscript{\textasteriskcentered}} & 0.89 & 0.39 \\
\lawaq & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{0.14\textsuperscript{\textdagger}} & 0.22 & 0.55 & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & 0.66 & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & 0.25 & 0.24 & 0.56 & 0.22 \\
\nadamp & 0.80 & 0.07 & 0.22 & 0.49 & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{0.90\textsuperscript{\textdagger}} & 0.88 & 0.94 & 0.85 & 0.60 & \textcolor{TUdark_light}{0.43\textsuperscript{\textdaggerdbl}} & \textcolor{TUdark_light}{0.74\textsuperscript{\textasteriskcentered}} & 0.80 & 0.47 \\
\sfadam & 0.67 & 0.05 & 0.13 & 0.41 & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & 0.57 & 0.92 & \B 0.57 & 0.78 & \textcolor{TUdark_light}{0.29\textsuperscript{\textdaggerdbl}} & \textcolor{TUdark_light}{0.61\textsuperscript{\textasteriskcentered}} & \B 0.33 & \B 0.12 \\
\sfprodigy & \textcolor{TUdark_light}{\texttt{NaN}} & \textcolor{TUdark_light}{\texttt{NaN}} & \textcolor{TUdark_light}{0.21\textsuperscript{\textdaggerdbl}} & \textcolor{TUdark_light}{0.65\textsuperscript{\textasteriskcentered}} & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{0.61\textsuperscript{\textasteriskcentered}} & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{0.40\textsuperscript{\textdagger}} \\
\pytorch \newline \textsc{Distr. Shampoo} & \B 0.65 & \B 0.03 & 0.15 & 0.22 & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{0.93\textsuperscript{\textdagger}} & \B 0.43 & 0.78 & 0.68 & 0.62 & 0.18 & 0.19 & 0.80 & 0.25 \\
\bottomrule
\end{tabularx}}



==> figs/runtimes_self_tuning.tex <==
{\renewcommand{\arraystretch}{1.25}\setlength{\tabcolsep}{4pt}\begin{tabularx}{0.98\textwidth}{>{\raggedright\arraybackslash}Xlglglgllgllglg}
\toprule
 & \multicolumn{2}{c}{\criteo} & \multicolumn{2}{c}{\fastmri} & \multicolumn{2}{c}{\resnet} & \vit & \multicolumn{2}{c}{\conformer} & \makecell{\textsc{Deep}\\ \textsc{Speech}} & \multicolumn{2}{c}{\ogbg} & \multicolumn{2}{c}{\wmt} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-8} \cmidrule(lr){9-10} \cmidrule(lr){11-11} \cmidrule(lr){12-13} \cmidrule(lr){14-15} & Base & H.O. & Base & H.O. & Base & H.O. & Base & Base & H.O. & Base & Base & H.O. & Base & H.O. \\
\midrule
\adamg & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} \\
\baseline & 0.75 & \B 0.07 & 0.22 & 0.51 & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & 0.95 & \B 0.94 & 0.92 & \B 0.65 & 0.46 & 0.69 & \B 0.84 & 0.59 \\
\textsc{NadamW}\newline \textsc{Sequential} & \textcolor{TUdark_light}{2.96\textsuperscript{\textdaggerdbl}} & \textcolor{TUdark_light}{0.57\textsuperscript{\textasteriskcentered}} & 0.27 & \B 0.44 & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & 1.58 & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{1.16\textsuperscript{\textdagger}} & 1.45 & 0.55 & 0.96 & \textcolor{TUdark_light}{2.36\textsuperscript{\textdaggerdbl}} & \textcolor{TUdark_light}{1.57\textsuperscript{\textasteriskcentered}} \\
\sfadam & \B 0.75 & 0.25 & \B 0.15 & 0.58 & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & \B 0.68 & 0.97 & \B 0.61 & 0.88 & \B 0.32 & \B 0.56 & 0.94 & \B 0.21 \\
\sinv & \textcolor{TUdark_light}{\texttt{NaN}} & \textcolor{TUdark_light}{\texttt{NaN}} & 0.49 & 0.87 & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{1.82\textsuperscript{\textdagger}} & 2.47 & \textcolor{TUdark_light}{1.35\textsuperscript{\textasteriskcentered}} & \textcolor{TUdark_light}{\texttt{inf}} & 2.32 & 0.46 \\
\sinvnum & \textcolor{TUdark_light}{\texttt{NaN}} & \textcolor{TUdark_light}{\texttt{NaN}} & 0.45 & 0.80 & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{\texttt{inf}} & \textcolor{TUdark_light}{2.55\textsuperscript{\textdagger}} & 2.21 & \textcolor{TUdark_light}{1.50\textsuperscript{\textasteriskcentered}} & \textcolor{TUdark_light}{\texttt{inf}} & 1.82 & 0.44 \\
\bottomrule
\end{tabularx}}



==> figs/speedups_external_tuning.tex <==
{\renewcommand{\arraystretch}{1.25}
\setlength{\tabcolsep}{4pt}
\begin{tabularx}{0.85\textwidth}{XS[table-format=2.2]}
\toprule
\textbf{Submission} & \textbf{Speed-up} \\
\midrule
\shampoosubshort & +27.87\% \\
\sfadam & +26.60\% \\
\caspr & +24.33\% \\
\generalizedadam & +10.89\% \\
\cycliclr & +10.67\% \\
\lawaq & +7.98\% \\
\nadamp & +3.37\% \\
\amos & +1.46\% \\
\rowcolor{TUgray_light}\baseline & -0.00\% \\
\lawaema & -9.17\% \\
\sfprodigy & -15.68\% \\
\bottomrule
\end{tabularx}
}


==> figs/speedups_self_tuning.tex <==
{\renewcommand{\arraystretch}{1.25}
\setlength{\tabcolsep}{4pt}
\begin{tabularx}{0.85\textwidth}{XS[table-format=3.2]}
\toprule
\textbf{Submission} & \textbf{Speed-up} \\
\midrule
\sfadam & +7.76\% \\
\rowcolor{TUgray_light}\baseline & -0.00\% \\
\nadamwseq & -92.44\% \\
\sinvnum & -157.67\% \\
\sinv & -168.63\% \\
\adamg & -294.16\% \\
\bottomrule
\end{tabularx}
}


==> figs/submissions_external_tuning.tex <==
{\renewcommand{\arraystretch}{1.3}
\setlength{\tabcolsep}{4pt}
\hyphenpenalty=10000\exhyphenpenalty=10000
\begin{tabularx}{0.98\textwidth}{@{}p{1.5cm}>{\raggedright}p{2.5cm}>{\raggedright}p{1.5cm}p{1.5cm}X@{}}
\toprule
\textbf{Submission} & \textbf{Authors} & \textbf{Institutions} & \textbf{Framework} & \textbf{Description} \\ \midrule
\makecell{\textsc{PyTorch}\\ \textsc{Distr.}\\ \textsc{Submission}} & Hao-Jun Shi, Tsung-Hsien Lee, Anna Cai, Shintaro Iwasaki, Wenyin Fu, Yuchen Hao, Mike Rabbat & Meta Platforms  & \pytorch & Based on the Distributed Shampoo algorithm of \citet{anil2020shampoo} with an implementation tailored to leverage PyTorch performance optimizations. See~\cite{shi2023distributeddataparallelpytorchimplementation} for details. The submission uses a list of five hyperparameter settings. \\
\makecell{\textsc{Schedule} \\ \textsc{Free}\\ \textsc{AdamW}} & Alice Yang, Aaron Defazio, Konstantin Mishchenko & Meta AI, Samsung AI  & \pytorch & A externally tuned version of \sfadam \citep{defazio2024road} with a list of five \hp configurations. \\
\makecell{\textsc{General-}\\ \textsc{ized}\\ \textsc{Adam}} & George Dahl, Sourabh Medapati, Zack Nado, Rohan Anil, Shankar Krishnan, Naman Agarwal, Priya Kasimbeg, Vlad Feinberg & Google  & \jax & Submission with an \adam-style update rule, tuning over the use of Nesterov acceleration and preconditioning. Essentially tuning over \adamw \citep{Kingma2015}, \nadamw, and \sgd \citep{Robbins1951} with or without momentum.\\
\cycliclr & Niccolò Ajroldi, Antonio Orvieto, Jonas Geiping & MPI-IS, ELLIS Institute Tübingen  & \pytorch & Revisits the work of \citet{Loshchilov2017} and \citet{smith2017cyclical}, coupling \nadamw \citep{Dozat2016,Loshchilov2019} with a cyclic learning rate scheduler. Each cycle involves a linear warmup phase for the LR, followed by cosine annealing. \\
\nadamp & George Dahl, Sourabh Medapati, Zack Nado, Rohan Anil, Shankar Krishnan, Naman Agarwal, Priya Kasimbeg, Vlad Feinberg & Google  & \jax & Uses \nadamw with an extra tunable hyperparameter $p$ enabling $p$th root of denominator inside \nadamw update rule instead of the default of $2$. \\
\rowcolor{TUgray_light}\baseline & &  & \jax &  Baseline using \nadamw \citep{Dozat2016,Loshchilov2019} and a linear learning rate warmup followed by a cosine decay \citep{Dahl2023AlgoPerf}. \\
\amos & Ran Tian & Google & \jax & Submission based on the \amos optimizer \citep{Tian2022} with a list of five \hp settings.\\
\makecell{\textsc{CASPR}\\ \textsc{Adaptive}} & Sai Surya Duvvuri, Inderjit S. Dhillon, Cho-Jui Hsieh & UT Austin, UCLA, Google  & \jax &  A submission based on \citep{Duvvuri2024} with a list of five \hp configurations.\\
\lawaq & Niccolò Ajroldi, Antonio Orvieto, Jonas Geiping & MPI-IS, ELLIS Institute Tübingen  & \pytorch & Employs Latest Weight Averaging \citep{izmailov2018swa,kaddour2022lawa} on top of \nadamw \citep{Dozat2016,Loshchilov2019}, maintaining a queue of previous model weights. The queue is periodically updated during training and passed to the competition API for evaluation. \\
\lawaema & Niccolò Ajroldi, Antonio Orvieto, Jonas Geiping & MPI-IS, ELLIS Institute Tübingen & \pytorch &  Similar to \lawaq but maintaining an exponential moving average of the model weights, which is updated periodically during training and returned to the competition API for evaluation. \\
\makecell{\textsc{Schedule}\\ \textsc{Free}\\ \textsc{Prodigy}} & Alice Yang, Aaron Defazio, Konstantin Mishchenko &  Meta AI, Samsung AI & \pytorch & Combining Schedule-free \citep{defazio2024road} with the \textsc{Prodigy} optimizer \citep{Mishchenko2024}. \\
\bottomrule
\end{tabularx}
}


==> figs/submissions_self_tuning.tex <==
{\renewcommand{\arraystretch}{1.3}
\setlength{\tabcolsep}{4pt}
\hyphenpenalty=10000\exhyphenpenalty=10000
\begin{tabularx}{0.98\textwidth}{@{}p{1.6cm}>{\raggedright}p{2.5cm}>{\raggedright}p{1.5cm}p{1.5cm}X@{}}
\toprule
\textbf{Submission} & \textbf{Authors} & \textbf{Institutions} & \textbf{Framework} & \textbf{Description} \\ \midrule
\makecell{\textsc{Schedule}\\ \textsc{Free}\\ \textsc{AdamW}} & Alice Yang, Aaron Defazio, Konstantin Mishchenko & Meta AI, Samsung AI & \pytorch & A self-tuning version of \sfadam \citep{defazio2024road} using a single \hp configuration.\\
\rowcolor{TUgray_light}\baseline & &  & \jax & Baseline using \nadamw, a linear learning rate warmup followed by a cosine decay, and a single hyperparameter point \citep{Dahl2023AlgoPerf}. \\
\makecell{\textsc{NadamW}\\ \textsc{Sequential}} & George Dahl, Sourabh Medapati, Zack Nado, Rohan Anil, Shankar Krishnan, Naman Agarwal, Priya Kasimbeg, Vlad Feinberg & Google & \jax & Uses \nadamw update rule and runs 3 fixed \hp points sequentially. The intention was for these to be the top 3 \hp points found at one third the self-tuning ruleset step budgets. \\
\textsc{Sinv6 75} & Abhinav Moudgil & Mila, Concordia University & \jax & A submission for a task-invariant learned optimizer meta-trained on small tasks. Uses $75\%$ of the number of steps as target in learned optimizer initialization.\\
\textsc{Sinv6} & Abhinav Moudgil & Mila, Concordia University & \jax & A submission for a task-invariant learned optimizer meta-trained on small tasks. \\
\textsc{AdamG} & Yijiang Pang & Michigan State University & \pytorch & A submission based on the \textsc{AdamG} optimizer \citep{Pang2024}. \\
\bottomrule
\end{tabularx}
}


==> figs/timing_jax_vs_pytorch.tex <==
{\renewcommand{\arraystretch}{1.25}
\setlength{\tabcolsep}{4pt}
\hyphenpenalty=10000\exhyphenpenalty=10000
\begin{tabularx}{0.6\textwidth}{XS[table-format=4]>{\columncolor{TUgray_vlight}}S[table-format=4]S[table-format=4]>{\columncolor{TUgray_vlight}}S[table-format=4]S[table-format=2]>{\columncolor{TUgray_vlight}}S[table-format=2]}
\toprule
\textbf{Workload} & \multicolumn{2}{c}{\textbf{\jax}} & \multicolumn{2}{c}{\textbf{\pytorch}} & \multicolumn{2}{c}{\textbf{Difference}} \\
\cmidrule(l){2-3} \cmidrule(l){4-5} \cmidrule(l){6-7}
                  & \text{Before}          & \text{After}          & \text{Before}            & \text{After}            & \text{Before}              & \text{After}             \\ \midrule
\criteo           & 127             & 136            & 213               & 122              & 68\%                & -10\%             \\
\fastmri          & 148             & 145            & 163               & 163              & 10\%                & 12\%              \\
\resnet           & 1047            & 1063           & 1174              & 1135             & 12\%                & 7\%               \\
\vit              & 1290            & 1378           & 1260              & 1253             & -2\%                & -9\%              \\
\conformer        & 1689            & 1445           & 1755              & 1407             & 4\%                 & -3\%              \\
\deepspeech       & 1047            & 875            & 1229              & 967              & 17\%                & 10\%              \\
\ogbg             & 306             & 399            & 398               & 445              & 30\%                & 12\%              \\
\wmt              & 804             & 782            & 972               & 792              & 21\%                & 1\%               \\ \bottomrule
\end{tabularx}
}


==> figs/workloads.tex <==
\begin{tabularx}{0.98\textwidth}{@{}XllllS[table-format=2.6]S[table-format=6.0]@{}}
	\toprule
                              &              &              &     &      & {Validation} & {\Runtime} \\ 
\textbf{Task} & \textbf{Dataset} & \textbf{Model} & \textbf{Loss} & \textbf{Metric} & \textbf{Target} & \textbf{Budget} \\ \midrule
Clickthrough rate \newline prediction  & \criteo      & \dlrmsmall   & CE  & CE   & 0.123735   & 7703    \\ \addlinespace
MRI reconstruction            & \fastmri     & \unet        & L1  & SSIM & 0.7344     & 8859    \\ \addlinespace
Image                         & \imagenet    & \resnetfifty & CE  & ER   & 0.22569    & 63008   \\
classification                &              & \vit         & CE  & ER   & 0.22691    & 77520   \\ \addlinespace
Speech                        & \librispeech & \conformer   & CTC & WER  & 0.085884   & 61068  \\
recognition                   &              & \deepspeech  & CTC & WER  & 0.119936   & 55506   \\ \addlinespace
Molecular property \newline prediction & \ogbg        & \gnn         & CE  & mAP  & 0.28098    & 18477   \\ \addlinespace
Translation                   & \wmt         & \transformer & CE  & BLEU & 30.8491    & 48151   \\ \bottomrule
\end{tabularx}

